Forty hours of declarative programming: Teaching Prolog at the Junior College Utrecht

This paper documents our experience using declarative languages to give secondary school students a first taste of Computer Science. The course aims to teach students a bit about programming in Prolog, but also exposes them to important Computer Science concepts, such as unification or searching strategies. Using Haskell's Snap Framework in combination with our own NanoProlog library, we have developed a web application to teach this course.

==> eptcsdata.tex <==
\providecommand{\firstpage}{50}
\providecommand{\publicationstatus}{M. Moraz\'an and P. Achten (Eds.): Trends in Functional \\ Programming in Education 2012 (TFPIE 2012).\\
EPTCS 106, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.106.4}{10.4204/EPTCS.106.4}}
\pdfoutput=1

